Searches for new phenomena in final states with leptons and jets using the ATLAS detector

The Standard Model is the most precise and consequential theory of science, yet it is not a complete account of all fundamental physics. Amongst its limitations, it lacks a coherent unification of quantum mechanics and gravity, and thus cannot resolve the large hierarchy gap between the weak and Planck scales. It does not explain neutrino masses or the evidence implying the existence of Dark Matter, nor does it provide a viable mechanism for baryogenesis sufficient to explain the observed matter-antimatter asymmetry in the Universe. Lastly, it is in tension with observations hinting toward charged Lepton Flavour Universality violation. These shortcomings indicate that physics beyond the Standard Model must exist. In this thesis, the ATLAS detector at the Large Hadron Collider is used to perform three distinct searches for New Physics. The first targets hypothetical, TeV-scale quantum black holes, which arise in extra-dimensional theories seeking to solve the hierarchy problem. Exploiting a unique feature of the model that strongly enhances the production rate with the collider centre-of-mass energy, and thereby permits a considerable increase in mass reach, it uses lepton+jet final states and sets the strongest limits on the model to date. The second tackles anomalies in lepton flavour by searching for heavy resonances that violate flavour conservation; targeting dilepton+$b$-jets final states, it complements previous inclusive results by directly addressing exclusive ones. The third targets Clockwork, periodic signatures of heavy graviton states appearing in extra-dimensional models. Performed in dielectron and diphoton final states, it establishes a new method to search for periodic signals using wavelet transformations with machine learning, and sets the best limits on the model.

==> preliminaries/epigraph.tex <==
\vspace*{\fill}
\begin{center}
\begin{minipage}{0.65\textwidth}
  \centering
  \itshape
  ``If you can look into the seeds of time,\\
  And say which grain will grow and which will not,\\
  Speak then to me, who neither beg nor fear\\
  Your favours nor your hate.''

  \bigskip
  \upshape\normalsize William Shakespeare\\
  \textit{Macbeth}, Act~I, Scene~3
\end{minipage}
\end{center}
\vspace*{\fill}

